GASP: A Gradient-Aware Shortest Path Algorithm for Boundary-Confined Visualization of 2-Manifold Reeb Graphs

Reeb graphs are an important tool for abstracting and representing the topological structure of a function defined on a manifold. We have identified three properties for faithfully representing Reeb graphs in a visualization: they should be constrained to the boundary, compact, and aligned with the function gradient. Existing algorithms for drawing Reeb graphs are agnostic to or violate these properties. In this paper, we introduce an algorithm to generate Reeb graph visualizations, called GASP, that is cognizant of these properties, thereby producing visualizations that are more representative of the underlying data. To demonstrate the improvements, the resulting Reeb graphs are evaluated both qualitatively and quantitatively against the geometric barycenter algorithm, using its implementation available in the Topology ToolKit (TTK), a widely adopted tool for calculating and visualizing Reeb graphs.

==> fig.duck.tex <==
\begin{figure}[!hbt]

    \begin{minipage}[m]{0.2\linewidth}
        \includegraphics[width=\linewidth]{figs/Evaluation-Examples/Reeb_Graph_Parameters/Ours/Color_Map/duck-y-180.png}
    \end{minipage}
    \hfill
    \begin{minipage}[m]{0.75\linewidth}
        \rotatebox{90}{\hspace{5pt} \tiny \textsf{Boundary Approach}}
        \subfloat[$S\mathbin{=}0.025$\label{fig:duck-c-0.025}]{\includegraphics[width=0.32\linewidth]{figs/Evaluation-Examples/Reeb_Graph_Parameters/Ours/CS/duck_y_boundary_0.025_None_180.png}}     
        \hfill
        \subfloat[$S\mathbin{=}0.05$\label{fig:duck-c-0.05}]{\includegraphics[width=0.32\linewidth]{figs/Evaluation-Examples/Reeb_Graph_Parameters/Ours/CS/duck_y_boundary_0.05_None_180.png}}
        \hfill
        \subfloat[$S\mathbin{=}0.1$\label{fig:duck-c-0.1}]{\includegraphics[width=0.32\linewidth]{figs/Evaluation-Examples/Reeb_Graph_Parameters/Ours/CS/duck_y_boundary_0.1_None_180.png}}        
        \hfill

        \rotatebox{90}{\hspace{5pt} \tiny \textsf{Interior Approach}}
        \subfloat[$B\mathbin{=}0.0$\label{fig:duck-i-0.00}]{\includegraphics[width=0.32\linewidth]{figs/Evaluation-Examples/Reeb_Graph_Parameters/Ours/Buffer/duck_y_interior_0.05_0_180.png}}
        \hfill
        \subfloat[$B\mathbin{=}0.025$\label{fig:duck-i-0.025}]{\includegraphics[width=0.32\linewidth]{figs/Evaluation-Examples/Reeb_Graph_Parameters/Ours/Buffer/duck_y_interior_0.05_0.025_180.png}}
        \hfill
        \subfloat[$B\mathbin{=}0.05$\label{fig:duck-i-0.05}]{\includegraphics[width=0.32\linewidth]{figs/Evaluation-Examples/Reeb_Graph_Parameters/Ours/Buffer/duck_y_interior_0.05_0.05_180.png}}        
    \end{minipage}

    \caption{The \texttt{duck} ($y$ function) model illustrating the effects of varying the (a-c)~\textit{contour spacing} for the boundary approach and the (d-f)~\textit{buffer size} for the interior approach with fixed contour spacing ($S\mathbin{=}0.05$).}
    \label{fig:varying_spacing_and_buffer}
\end{figure}

